Functorial Question Answering

Distributional compositional (DisCo) models are functors that compute the meaning of a sentence from the meaning of its words. We show that DisCo models in the category of sets and relations correspond precisely to relational databases. As a consequence, we get complexity-theoretic reductions from semantics and entailment of a fragment of natural language to evaluation and containment of conjunctive queries, respectively. Finally, we define question answering as an NP-complete problem.

==> eptcsdata.tex <==
\providecommand{\firstpage}{84}
\providecommand{\publicationstatus}{John Baez and Bob Coecke (Eds.): Applied Category Theory 2019\\
EPTCS 323, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.323.6}{10.4204/EPTCS.323.6}}


==> header.tex <==
%!TEX root = discocat-act2019.tex

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\RequirePackage{doi}
\usepackage{hyperref}

\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{mathrsfs}
\usepackage{braket}
\usepackage{physics}
\usepackage{tikz}
\usepackage{newtxtext}
\usepackage{newtxmath}
\usetikzlibrary{matrix,arrows,decorations.pathmorphing}
\usetikzlibrary{decorations.markings}

\newcommand{\s}{\enspace}
\newcommand{\sub}{\subseteq}
\newcommand{\size}[1]{\left\vert{#1}\right\vert}
% \renewcommand{\tt}[1]{\mathtt{#1}}
% \renewcommand{\bf}[1]{\mathbf{#1}}
% \renewcommand{\sc}[1]{\textsc{#1}}
\renewcommand{\cal}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\phi}{\varphi}
\newcommand{\xto}[1]{\xrightarrow{#1}}
\newcommand{\injects}{\xhookrightarrow{}}
\newcommand{\from}{\leftarrow}
\newcommand{\rel}[3]{#1 \sub #2 \times #3}
\newcommand{\graph}[2]{#1 \sub #2^2}
\newcommand{\B}{\bb{B}}
\newcommand{\N}{\bb{N}}
\newcommand{\Z}{\bb{Z}}

\newtheorem{draft}{DRAFT}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{conjecture}[definition]{Conjecture}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{example}[definition]{Example}
\newtheorem{remark}[definition]{Remark}

\usepackage{tabularx,environ}
\makeatletter
\newcommand{\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand{\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand{\problemoutput}[1]{\gdef\@problemoutput{#1}}% Store problem question
\NewEnviron{problem}{
  \problemtitle{}\probleminput{}\problemoutput{}% Default input is empty
  \BODY% Parse input

   \@problemtitle
  \par\addvspace{.5\baselineskip}
  \noindent
  \begin{tabularx}{\textwidth}{@{\hspace{\parindent}} l X c}
    \textbf{Input:} & \@probleminput \\% Input
    \textbf{Output:} & \@problemoutput% Question
  \end{tabularx}
  \par\addvspace{.5\baselineskip}
}

